Quantum mechanical potentials exactly solvable in terms of higher hypergeometric functions. I: The third-order case

We present a new six-parameter family of potentials whose solutions are expressed in terms of the hypergeometric functions 3F2, 2F2 and 1F2. Both the scattering data and the bound states of these potentials are explicitly computed and the peculiar properties of the discrete spectrum are depicted in a suitable phase diagram. Our starting point is a third-order formal eigenvalue equation of the hypergeometric type (with a suitable solution known) which is transformed to the Schr\"odinger equation by applying the reduction of order technique as the crucial first step. The general preconditions allowing for the reduction to Schr\"odinger form of an arbitrary eigenvalue equation of higher order, are discussed at the end of the article, and two universal features of the potentials arising this way are also stated and discussed. In this general scheme the Natanzon potentials are the simplest special case, those presented here the next ones, and so on for potentials arising from equations of fourth or higher order.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%\bar + kati %%%%%%%%%%%%%%%%
\def\Ebar{\kern2.4pt\overline{\hbox to 6.2pt{\kern-2.4pt $E$}}}
\def\Abar{\kern2.4pt\overline{\hbox to 6.2pt{\kern -2.4pt $A$}}}
\def\Bbar{\kern2.4pt\overline{\hbox to 6.2pt{\kern -2.4pt $B$}}}
\def\Vbar{\kern2.4pt\overline{\hbox to 6.2pt{\kern-2.4pt $V$}}}
\def\VBar{\kern2pt \overline{\hbox to 5pt{\kern-2.4pt $V$}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%ANAFORES (Kefalaio, paragrafos, selida)%%%%%%%%%%%%%%
%% \item Επικαλεστείτε τη θεωρία των μετασχηματισμών συμμετρίας
%% του κεφαλαίου \ref{ch:generalformalism} (παράγραφος \ref{subsec:transspin},
%% σελ.\ \pageref{eq:dimito}) για να προβλέψετε το δεύτερο μέλος
%% των ακόλουθων μετέωρων εξισώσεων

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FOOTNOTE INTO SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%\section[%
%%% H periptwsh \textlatin{Pauli}]{%
%%% H periptwsh \textlatin{Pauli}\footnote{some footnote text\ldots}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%\section[%
%%% H periptwsh \textlatin{Pauli}]{%
%%% H periptwsh \textlatin{Pauli}\footnotemark}
%%%\footnotetext{this is some footnote text\ldots}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%ALLAGH BOXWIDTH (COLORBOX)%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% \fboxsep 8pt
%%%%%%%%%%%% \newlength\boxwidth
%%%%%%%%%%%% \boxwidth=117mm %%%%\textwidth
%%%%%%%%%%%% \advance\boxwidth -\fboxsep
%%%%%%%%%%%% \advance\boxwidth -\fboxsep

%%%% Gia thn grammh me to galazio fonto, 8eleis prin apo to
%%%% \begin{document} mia dhlwsh tou typou:
%%%% 
%%%% \def\blueboxtext#1{%
%%%% \vskip2.0pt%
%%%% \noindent%
%%%% \hbox to 0pt{\color{lightblue}\rule[-5.0pt]{\textwidth}{18pt}}%
%%%% \makebox[\textwidth][c]{#1}
%%%% \vskip2.0pt
%%%%  }
%%%%  Meta mporeis na to xrhsimopoihseis etsi:
%%%%  \blueboxtext{Kapoio keimeno...}
%%%% (Mporeis na pai3eis me tis diastaseis ths grammhs mexri na
%%%% ikanopoih8eis me thn topo8ethsh tou keimenou panw sthn grammh.)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%\lquote\lquote
%Schr\"{o}dinger
%$^.$
%{·}
%{Ά}
%{ΐ}
%{ΰ}

%%% \def\PIkato{\displaystyle{\Pi\atop{\scriptstyle (k\ne j)}}}
%% \def\PIkato{\displaystyle{\Pi\limits_{(k\ne j)}}}
\def\PIkato{\begin{array}{c}\Pi\\ \Nonono{\scriptstyle (k\ne j)}%%%%
\end{array}}

\def\MHDE{{\Large 0}}
\def\vsk{\vskip3pt}
\def\vvsk{\vskip5pt}
\def\RULE{\hrule width 126mm height 0.4pt}
\def\RuLe{\hrule width 110mm height 0.4pt}
\def\RULe{\hrule width 98mm height 0.4pt}
\def\rULE{\hrule width 70mm height 0.4pt}

%%%%%   BARES DIAFORES !!!!!!!!!!!!!!!!!!!!!!!!!!!!
\def\Ebar{\kern2.4pt\overline{\hbox to 6.2pt{\kern-2.4pt $E$}}}
\def\Abar{\kern2.4pt\overline{\hbox to 6.2pt{\kern -2.4pt $A$}}}
\def\Bbar{\kern2.4pt\overline{\hbox to 6.2pt{\kern -2.4pt $B$}}}
\def\Pbar{\kern2.4pt\overline{\hbox to 6.2pt{\kern -2.4pt $P$}}}

%%%%% \section{Θεωρία διαταραχών εκφυλισμένης στάθμης}
%%%%% \markright{I.2. ΘΕΩΡΙΑ ΔΙΑΤΑΡΑΧΩΝ ΕΚΦΥΛΙΣΜΕΝΗΣ ΣΤΑΘΜΗ}
%%%%% \addcontentsline{toc}{section}{ΘΕΩΡΙΑ ΔΙΑΤΑΡΑΧΩΝ ΕΚΦΥΛΙΣΜΕΝΗΣ ΣΤΑΘΜΗ}


\setlength\arraycolsep{2pt}

\def\tbsl{\bf\em}
%%%%% \penalty-50


%%%%% \,{\buildrel {\scriptstyle <}\over{\scriptstyle\simeq}}\,
%%%%%   \; \raisebox{-5pt}{$\stackrel{\textstyle =}
%%%%%   {\scriptscriptstyle r\sim\infty}$}\;
%%%%%  $\bigcirc\kern-.323cm{\scriptstyle A}\,$
%%%%% \; \sim\hskip-16pt\raisebox{-5pt}{$\scriptscriptstyle r\to\infty$}\;
%%%%%%%  \fontseries{b}\fontshape{sc}\selectfont
%%%%%%% \fontseries{m}\fontshape{sc}\selectfont
%%%%\noindent \hangindent=12pt \hangafter=1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\,
%%%%\raisebox{-5pt}{$\stackrel{\textstyle\longrightarrow}
%%%%  {\scriptscriptstyle r\to\infty}$}\;


%%%% \,\, \mathop{=}\limits_{\mbox{ορ}}\,\,

\def\ratel{{ \raisebox{2.1pt}{\kern 1pt .}}}
\def\rakom{{ \raisebox{2.1pt}{\kern 1pt ,}}}
\def\IF{{\mathrm{\scriptsize if}}}
\def\erf{{\mathrm{erf}}}
%%%%\def\sp{{\mathrm{\scriptsize sp}}}
\def\sp{{\mathrm{\scriptscriptstyle sp}}}
%%%%\def\FI{{\mathrm{\scriptsize fi}}}
\def\kefalis{\textlatin{$x$}}
\def\KEFAL{$\phi={1\over 2}\alpha$\kefalis$^2+\beta$\kefalis$+\gamma$}
\def\FI{{\mathrm{fi}}}
\def\SC{{\mathrm{sc}}}
\def\sech{{\mathrm{sech}}}
\def\sign{{\mathrm{sign}}}
\def\Or{{\mbox{\scriptsize ορ}}}
%%%%\def\scc{{\mathrm{\scriptsize sc}}}
\def\scc{{\mathrm{sc}}}
\def\LS{\textlatin{\rm LS}}
\def\IS{\textlatin{\rm IS}}
\def\Jm{\textlatin{\rm Jm}\,}
\def\I{\textlatin{\rm I}}
%%%%\def\S{\textlatin{\rm S}}
\def\SYN{\hbox{\tenrm +}}
\def\nosm{\noalign{\smallskip}}
\def\nomed{\noalign{\medskip}}
\def\nobig{\noalign{\bigskip}}
\def\nono{\noalign{\vskip-10pt}}
\def\Nonono{\noalign{\vskip-6pt}}
\def\lign{\noalign{\vskip-.3cm}}
\def\NONO{\noalign{\vskip-3.5pt}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\def\upr{\uparrow\uparrow}
\def\updr{\uparrow\downarrow}

\def\noab{\noalign{\bigskip}}
\def\noa{\noalign{\medskip}}
\def\noai{\noalign{\smallskip}}
\def\noaii{\noalign{\vskip1pt}}

\def\bbakk{\vskip-5pt}
%%\renewcommand\BAK{\vspace-3cm}
%\def\backk{{\noalign{\vskip-.5pt}}}    \lineskip=0pt

\def\arx{\mbox{\scriptsize αρχ}}
\def\arxikh{\mbox{\scriptsize αρχική}}
\def\tel{\mbox{\scriptsize τελ}}
\def\telikh{\mbox{\scriptsize τελική}}
%%%%\def\diakrisi{\tiny{\mbox{διακρίσιμα}\atop\mbox{σωματίδια}}}
\def\diakrisi{{\mbox{\scriptsize διακρίσιμα}\atop\mbox{\scriptsize σωματίδια}}}
%%%%\def\midiakrisi{\tiny{\mbox{μη διακρίσιμα}\atop\mbox{σωματίδια}}}
\def\midiakrisi{{\mbox{\scriptsize μη διακρίσιμα}\atop\mbox{\scriptsize σωματίδια}}}
\def\uemel{\mbox{\scriptsize θεμελιώδης}}
\def\ket{\hbox{\textlatin{ket}}\,}
%%%% \def\olx{\mbox{\matrix{\mathrm{\mbox{όλος\ ο}}\hfill\cr
\def\olx{{\mbox{\tiny όλος ο}\atop\mbox{\tiny χώρος}}}
%%%% \noalign{\vskip-5pt}
%%%% \mbox{\mathrm{\mbox{χώρος}}\hfill\cr}}}}


\def\oooo{{\matrix{\hbox{\sevenesl j}\hbox{\sevenrm =3/2}\hfill\cr
\noalign{\vskip-5pt}
\hbox{\sevenesl m}_j\hbox{\sevenrm =3/2}\hfill\cr}}}

\def\Oooo{{\matrix{{\scriptstyle\ell}\hbox{\sevenrm =1}\hfill\cr
\noalign{\vskip-5pt}
\hbox{\sevenesl m}\hbox{\sevenrm =1}\hfill\cr}}}

\def\oooO{{\matrix{\hbox{\sevenesl j}\hbox{\sevenrm =3/2}\hfill\cr
\noalign{\vskip-5pt}
\hbox{\sevenesl m}_j\hbox{\sevenrm =1/2}\hfill\cr}}}

\def\OooO{{\matrix{{\scriptstyle\ell}\hbox{\sevenrm =1}\hfill\cr
\noalign{\vskip-5pt}
\hbox{\sevenesl m}\hbox{\sevenrm =0}\hfill\cr}}}

%%%%%%%%%% \def\kpE{
%%%%%%%%%% {\matrix{\hbox{\sevenesl k=p/}{\scriptstyle\hbar}\hfill\cr
%%%%%%%%%% \noalign{\vskip-5pt}
%%%%%%%%%% \hbox{\sevenesl ω=E/}{\scriptstyle\hbar}\hfill\cr}}}

\def\kpE{
\begin{eqnarray*}
k &=& p/\hbar \\
\noalign{\vskip-5pt}
\omega &=& E/\hbar
\end{eqnarray*}}

\def\anis{{\matrix{\hbox{\sevenesl m}\cr
\noalign{\vskip-5pt}
\hbox{{\sevenrm(}\sevenesl m}
  {\scriptstyle\ne}\hbox{\sevenesl n{\sevenrm )}}\cr}}}


\def\eept{{\matrix{\hbox{\sevenesl s}\hbox{\sevenrm =1}\hfill\cr %%%\backk %%%%
\noalign{\vskip-5pt}
\hbox{\sevenesl μ} \hbox{\sevenrm =0}\hfill\cr}}} 

\def\matr{{\eept}}

\def\eeptt{{\matrix{\hbox{\sevenesl s}\hbox{\sevenrm =1}\hfill\cr %%%\backk %%%%
\noalign{\vskip-5pt}
\hbox{\sevenesl μ} \hbox{\sevenrm =-1}\hfill\cr}}}
\def\mmatr{{\eeptt}}

\def\anoi{«}
\def\klei{»$\,\,$}
\def\klein{»}

\font\eva=bbm10
\font\beva=bbmbx10
\font\seva=bbmsl10
\font\eveva=bbm7
\font\Eva=bbm12

\def\alr{|\alpha\rangle}
\def\all{\langle\alpha |}
\def\nra{|n\rangle}

\def\pso{\psi^{(0)}}
\def\psena{\psi^{(1)}}
\def\psr{|\psi\rangle}
\def\psl{\langle\psi |}

\def\phr{|\phi\rangle}
\def\phl{\langle\phi |}

\def\nra{|n\rangle}


\def\ar{\langle}
\def\de{\rangle} %%%%%%%%%%%%%%%%%%%%kkkkkk


\def\adag{a^{\dagger}}
%\def\lacksq{{\footnotesize{$\blacksquare$}}}
\def\blacksq{{\tiny{$\blacksquare$}}}
%%%%% \def\OR{\; {\buildrel {\mbox{\tiny ορ}} \over =}\; }
%%%%% \def\OR{\; {$\stackrel{=}{\mbox{\tiny ορ}}}}
\def\ROOO{\,\, \mathop{=}\limits_{\mbox{\tiny ορ}}\,\,}
\def\OR{\raisebox{-.10cm}{$\;\stackrel{=}{\mbox{\tiny ορ}}\;$}}
\def\DEF{\raisebox{-.11cm}{$\;\stackrel{=}{\mbox{\tiny \textlatin{def}}}\;$}}
\def\CNOT{\;\resizebox{.85cm}{.15cm}{$\longrightarrow$} \hskip-.83cm%%%
\raisebox{.25cm}{${\scriptscriptstyle{\mathrm{CNOT}}}$}\;\;}
%%%% \def\CNOT{\resizebox{.95cm}{.15cm}{$\longrightarrow$} \hskip-.95cm%%%
%%%% \raisebox{.25cm}{${\scriptstyle{\mathrm{CNOT}}}$}}
\def\cnot{\hbox{\textlatin{CNOT}}}
%%% \def\Z2{{\raisebox{-.15cm}{$\;\stackrel{=}{\scriptstyle (Z=2)}\;$}}}
\def\IN{{\hbox{\textlatin{\tiny in}}}}
\def\artios{\,{\mbox{\tiny άρτιος}}}
\def\perittos{\,{\mbox{\tiny περιττός}}}
\def\BULLET{\Huge{\bullet}}
\def\ARROW{\Huge{\Downarrow}}
\def\ELG{$\langle$}
\def\XXLLAA{\Huge\langle}

\def\blasq{{\scriptstyle {\blacksquare}}}

%\medskip
%\bigskip
%\hangindent=.55cm \hangafter=1
%\noindent
%{\twbsl 1.$\,\,$Αλγεβρική θεωρία της στροφορμής}
%\def\leftheadline{\vbox{\leftline{{\eigr\folio}\hfill
%\sevenh ΘΕΩΡΙΑ ΤΗΣ ΣΤΡΟΦΟΡΜΗΣ ΚΑΙ ΤΟ ΑΤΟΜΟ ΤΟΥ ΥΔΡΟΓΟΝΟΥ}\headrule}}
%\def\rightheadline{\vbox{\rightline{\sevenh
%ΑΛΓΕΒΡΙΚΗ ΘΕΩΡΙΑ ΤΗΣ ΣΤΡΟΦΟΡΜΗΣ\hfill{\eigr\folio}}\headrule}}
%\voffset=2\baselineskip
%
%\medskip
%\hangindent=.75cm \hangafter=1
%{\noindent\elevenbsl
%1.1.$\,\,$Αλγεβρικός υπολογισμός των ιδιοτιμών.
%Οι τελεστές αναβίβασης και καταβίβασης}


%\font\eigr
%\long\def\FOOTNOTE#1#2{{\baselineskip=9pt
%  \setbox\strutbox=\hbox{\vrule height 7pt depth 2pt width 0pt} %
%  \eigr
%\everypar{\hangindent=\parindent  %
%\footnote{#1}{#2}\everypar{}}} %


%\vbox to 8.4truecm{\centerline
%{\psfig{file=/home/sofia/SXETIKOTHTA/SXET_eps/S1.eps,height=8.4truecm}}}
%\bigskip
%\centerline{\sl Σχήμα 1}

\def\nopt{\noalign{\vskip2.pt}}

\def\inc{\textlatin{\rm inc}}
\def\Newton{\textlatin{\rm Newton}}
\def\Stark{\textlatin{\rm Stark}}
\def\Born{\textlatin{\rm B}}

\def\GGamma{{\it\Gamma}}
\def\GAM{{\scriptscriptstyle\mathit\Gamma}}
%%%%% \def\GGGamma{{\scriptsize\mbox{\em Γ}}}
%%%%% \def\GGGamma{\mbox{\textgreek{\scriptstyle\em Γ}}}
\def\Vtt{{\mathtt V}}
\def\thetab{\bscal\theta}
\def\rhob{\bscal\rho}
\def\taub{\bscal\tau}
\def\sigmab{\bscal\sigma}
\def\lambdab{\bscal\lambda}
\def\deltab{\bscal\delta}
\def\psib{\bscal\psi}
\def\phib{\bscal\phi}
\def\ellb{\bscal\ell}
\def\ellbs{{\mbox{\footnotesize{\bscal\ell}}}}
\def\mub{{\bscal\mu}}
\def\pib{{\bscal\pi}}
\def\mubs{\footnotesize{\bscal\mu}}
\def\bomega{{\bscal\omega}}
\def\mubs{{\mbox{\footnotesize{\bscal\mu}}}}

\def\cm{\mathrm{cm}}
\def\He{\mathrm{He}}
\def\Li{\mathrm{Li}}
\def\Be{\mathrm{Be}}
\def\Ze{\mathrm{Ze}}


\def\hs{{\hskip7pt}}
%%%%\def\cl{{\mathrm{\scriptsize cl}}}
\def\cl{\mathrm{cl}}
\def\ol{{\scriptsize\mbox{ολ}}}
\def\b2{\mbox{\sevenbf 2}}
\def\bG{\mbox{\tenbsl Γ}}
\def\SS{{\mathrm S}}
\def\AAA{{\mathrm A}}
\def\HH{\mbox{\tiny H}}
%%%% \def\RR{\mbox{\tiny R}}
%%%% \def\RR{\mathop{\rm R}}
\def\RR{\mathrm{R}}
\def\LL{\mathrm{L}}
%%%%\def\Cooper{{\mathrm C}}
\def\NN{{\mathop{\rm N}}}
\def\BB{\mathop{\rm B}}
\def\local{\mathop{\rm local}}
\def\pert{\mathop{\rm pert.}}
\def\Zeeman{\mathop{\rm Zeeman}}
\def\orisma{{\mbox{\tiny ορ}}}
%%%% \def\TT{\mbox{\tiny T}}
%% \def\Bohr{\mathop{\rm B}}
\def\Bohr{\textlatin{\rm B}}
\def\TT{\mathop{\rm T}}
\def\ddyo{{\mbox{\footnotesize\tt 2}}}
\def\nnn{{\mbox{\footnotesize\tt n}}}
\def\at{\mbox{\textgreek{\scriptsize ατ}}}
\def\pyrhna{\mbox{\textgreek{\scriptsize πυρήνα}}}
\def\prin{\mbox{\textgreek{\scriptsize πριν}}}
\def\meta{\mbox{\textgreek{\scriptsize μετά}}}

%\item{}$\quad\,\,$
\def\te{$^.\,\,\,$}
\def\CC{\mbox{\sevenrm C}}
\def\UU{\mbox{\sevenrm U}}
\def\VV{\mbox{\sevenrm V}}
\def\YY{\mbox{\sevenrm Y}}
\def\XX{\mbox{\sevenrm X}}
\def\Alf{\mbox{\sevenrm A}}
\def\Bt{\mbox{\sevenrm B}}
\def\CE{\mbox{\sevenrm C}}
\def\wH{\widehat{H}}
\def\mi{\mbox{\bf μ}}
\def\xxi{\mbox{\bf χ}}
\def\xikef{{\scriptscriptstyle x}}
\def\ro{\bar{\mbox{\rm r}}}
\def\piksv{{\vspace*-9pt}}
\def\piksV{{\vskip*-9pt}}
\def\piksh{{\hspace*-3mm}}
\def\VVVVVVV{{\piksv{\setlength{\unitlength}{2mm}
\begin{picture}(1,1)
\put(0,0){\line(1,0){1}}
\end{picture}}\piksh}}
\def\LINE{\VVVVVVV}
%%%%% \def\zzZ{{\large{\bar{K}}}}
\def\ENIL{\rule[9pt]{2.2mm}{0.4pt}\!\!\!\!\!}
%%% \def\VVRRULE{{\COL\rule[9pt]{2mm}{1.2cm}}}
\def\Bara{\ENIL}
%\def\Af{\,\,{^{^{\bar}}}\!\;\!\!\!\!\mbox{\elerm A}}
\def\Af{^{^{\bar}}{\mbox{\elerm A}}}
\def\Ra{\bar{\mbox{\elerm R}}}
\def\roi{\bar{\mbox{\rm r}}_{\mbox{\sevenrm i}}}
\def\ros{\bar{\mbox{\rm r}}_{\mbox{\sevenrm s}}}
\def\roc{\bar{\mbox{\rm r}}_{\mbox{\sevenrm c}}}
\def\Thet{\mbox{\ninesl Θ}}
\def\Th{\mbox{\sevenesl Θ}}
\def\Delt{\mbox{\ninesl Δ}}
\def\Dela{\mbox{\sevenesl Δ}}
%\def\Deltat{\mbox{\sl D}}
\def\Pit{\mbox{\ninesl Π}}
\def\Phit{\mbox{\ninesl Φ}}
\def\Pip{\mbox{\sl Π}}
\def\Thetat{\mbox{\sl Θ}}
\def\Deltat{\mbox{\sl Δ}}
\def\Pita{\mbox{\sl Π}}
\def\Phita{\mbox{\sl Φ}}
\def\bcal#1{\mbox{$\textfont1=\boma #1$}}
\def\bscal#1{\mbox{$\textfont1=\boit #1$}}
\def\vl{\vrule width 12.6truecm height 1pt
}
%
\def\itemitemitem{\par\indent\indent\hangindent3\parindent\textindent}
%
\def\bbill{{\eightpoint{$\bullet$}}}
\def\bil{\bbill}
\def\ddbi{{\scriptscriptstyle\bullet}}
\def\bbil{\raise5pt\hbox{\scriptscriptstyle\bullet}}
%
% david: commented out:
%
%%%%\chardef\ll="AB
%%%%\chardef\gg="BB
%
%overleftrightarrow
%
\catcode`\@=11
\def\leftrightarrowfill{$\m@th\mathord\leftarrow\mkern-6mu%
  \cleaders\hbox{$\mkern-2mu\mathord-\mkern-2mu$}\hfill
    \mkern-6mu\mathord\rightarrow$}
\def\overleftrightarrow#1{\vbox{\ialign{##\crcr
        \leftrightarrowfill\crcr\noalign{\kern-\p@\nointerlineskip}
        $\hfil\displaystyle{#1}\hfil$\crcr}}}
%
\font\bsym=cmbsy10
\def\bnabla{\hbox{$\textfont2=\bsym \nabla$}}
%
\def\castok#1{\leavevmode\quad\qquad{\vrule\vtop{\vbox{\hrule\kern5pt
        \hbox{\vphantom{\rm/}\quad{\rm#1}\quad}}
      \kern5pt\hrule}\vrule}\quad} % control sequence token
%

\def\cstok#1{\leavevmode\qquad{\vrule\vtop{\vbox{\hrule\kern5pt
        \hbox{\vphantom{\rm/}\quad{\rm#1}\quad}}
      \kern5pt\hrule}\vrule}\qquad} % control sequence token
%
\newdimen\headrulewidth
\newdimen\headwidth
\headrulewidth 0.4pt
\headwidth 12.6truecm
\def\headrule{\vskip 6pt \hrule height \headrulewidth  width \headwidth }
\def\boxtext#1{%
\vbox{%
\hrule
\medskip
\hbox{\strut \vrule{} {\bf #1} \vrule}
\medskip
\hrule
}
}
\def\makeheadline{\vbox to 0cm{\vskip-26pt
  \line{\vbox to 8.5pt{}\the\headline}\vss}\nointerlineskip}
\def\sqr#1#2{{\vcenter{\vbox{\hrule height.#2pt
        \hbox{\vrule width.#2pt height#1pt \kern#1pt
          \vrule width.#2pt}
        \hrule height.#2pt}}}}
%Define d with bar
\def\dbar{\ {\mathchar'26\mkern-12mud}}
%Define int with slash
%\def\sint{\ {\mathchar'26\mkern-12mud}}
%
\def\boxtext#1{%
\vbox{%
\hrule
\hbox{\strut \vrule{} {\bf #1} \vrule}
\hrule
}
}
\def\makeheadline{\vbox to 0cm{\vskip-26pt
  \line{\vbox to 8.5pt{}\the\headline}\vss}\nointerlineskip}
\def\sqr#1#2{{\vcenter{\vbox{\hrule height.#2pt
        \hbox{\vrule width.#2pt height#1pt \kern#1pt
          \vrule width.#2pt}
        \hrule height.#2pt}}}}
%%% \def\gray#1#2{\noindent{{\special{ps:gsave #1 setgray}{\huge #2}
%%%    \special{ps:grestore}}}}
\def\square{\mathchoice\sqr67\sqr67\sqr{4.1}5\sqr{3.5}5}
\def\bulle{\vrule height 1.6ex width 1.6ex depth -.1ex }
\def\squar{\mathchoice\sqr34\sqr34\sqr{2.1}3\sqr{1.5}3}
\def\nit{\mathop{\rm int}\nolimits}
\def\pert{\mathop{\rm pert}\nolimits}
\def\var{\mathop{\rm var}\nolimits}
\def\mol{\mathop{\rm mol}\nolimits}
%%%%%%%%%%%%%%%\def\nb #1{{\rm{\bf #1}}}
\def\nb #1{{\mbox{\boldmath${#1}$}}}
\def\nbs #1{{\mbox{\scriptsize\boldmath${#1}$}}}
\def\nbss #1{{\mbox{\boldmath${#1}$}}}
\def\bolds{\boldsymbol}
\def\calE{\bolds{\cal E}} %%%%%%%%%%%%%%%% FOOTNOTE
\def\calA{\bolds{\cal A}}
\def\calPi{\bolds{\Pi}}
\def\calpi{\bolds{\pi}}
\def\bok{{\boldsymbol k}}
\def\boq{{\boldsymbol q}}
\def\bocdot{{\hskip1pt\boldsymbol\cdot}}
\def\bor{{\boldsymbol r}}
\def\ns #1{{\rm{\sl #1}}}
\def\dint #1{\!\!\int\limits_{\ \ #1}\!\!\int}
\def\ddint #1{\!\!\!\int\limits_{\ \ #1}\!\!\!\int}
\def\tint #1{\!\!\int\!\!\int\limits_{\ #1}\!\!\int}
\def\ttint #1{\!\!\!\int\!\!\!\int\limits_{\ \ #1}\!\!\!\int}
\def\Im{\mathop{\rm Im}}
\def\Re{\mathop{\rm Re}}
\def\exp{\mathop{\rm exp}\nolimits}
\def\csc{\mathop{\rm csc}\nolimits}
\def\div{\mathop{\rm div}\nolimits}
\def\curl{\mathop{\rm curl}\nolimits}
\def\grad{\mathop{\rm grad}\nolimits}
\def\opt{\mathop{\rm opt}\nolimits}
\def\rot{\mathop{\rm rot}\nolimits}
%
%Cases witout {
%
\def\Cases#1{\vcenter{\normalbaselines\m@th
   \ialign{$##\hfil$&\quad##\hfil\crcr#1}}}
%
%Mixed box
%
\def\Mboxit#1{\vbox{\hrule\hbox{\vrule\kern10pt
      \vbox{\kern-2pt#1\kern3pt}\kern15pt\vrule}\hrule}}
%
%mixed box
%
\def\mboxit#1{\vbox{\hrule\hbox{\vrule\kern20pt
      \vbox{\kern10pt#1\kern-12pt}\kern20pt\vrule}\hrule}}
%
%Single equation box
%
\def\sboxit#1{\vbox{\hrule\hbox{\vrule\kern20pt
      \vbox{\kern-3pt#1\kern-10pt}\kern20pt\vrule}\hrule}}
%
%SSingle equation box
%
\def\ssboxit#1{\vbox{\hrule\hbox{\vrule\kern20pt
      \vbox{\kern-10pt#1\kern-10pt}\kern20pt\vrule}\hrule}}
%
%Multiple line box
%
\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern20pt
      \vbox{\kern-10pt#1\kern-8pt}\kern20pt\vrule}\hrule}}
%
% One line box
%
\def\boxi#1{\vbox{\hrule\hbox{\vrule\kern20pt
      \vbox{\kern-4.5pt#1\kern10pt}\kern20pt\vrule}\hrule}}
%
%Macros for harpoon
%
\def\m@th{\mathsurround=0pt }
\def\rightharpoonupfill{$\m@th \mathord- \mkern-6mu
  \cleaders\hbox{$\mkern-2mu \mathord- \mkern-2mu$}\hfill
  \mkern-6mu \mathord\rightharpoonup$}
\def\harp#1{\vbox{\ialign{##\crcr
  \rightharpoonupfill\crcr\noalign{\kern-1pt\nointerlineskip}
  $\hfil\displaystyle{#1}\hfil$\crcr}}}

%
%Macro for phantom one char
%
\def\ph{\phantom{-}}
%
%Column formatting TeX macro
%
\def\colmac #1 #2 #3 #4 {% #1 for horizontal size of col 1 #2 the same for
% col 2 and #3 #4 is the text for first and second col.
%e.x. colmac {6} {0} {<text>} {<text>} for a white column the text is \hfil
\setbox0=\vbox{\hsize=#1 #3}
\setbox2=\vbox{\hsize=#2 #4}
\line{\box0\hfil\box2}
}
%Macros for quota
\newdimen\quotehang \setbox0=\hbox{`} \quotehang=\wd0
\newskip\zzz \def\allowhyphens{\nobreak\hskip\zzz}
\def\rquote{'\kern-\quotehang\kern\quotehang}
\def\lquote{\ifhmode\kern\quotehang\vadjust{}\else\leavevmode\fi \kern-\quotehang`\allowhyphens}
%
\def\llq{\lquote\lquote}
\def\rrq{\rquote\rquote}

%%%%%%%%%% ME GRAMMH PANO KAI KATO %%%%%%%%%%%%%%%%%%%%
%%% \begin{array}{cc}
%%% \def\elur{\rule{3.73cm}{.4pt}}
%%% \def\UUUU{\shortmid\hspace{-.135cm}\lower.5pt\hbox{$\elur$}%%
%%% \hspace{-.138cm}\shortmid}
%%% \hspace{5.4cm}\rotatebox{180}{$\UUUU$} \\
%%% \lign
%%% {\cal R}=\big|r(k)\big|^2\! = r(k)r^*(k)
%%% = \displaystyle{\sin^2\pi L\over\pi^2}\,
%%% \Gamma(-w)\Gamma(1+w^*) \Gamma(-w^*)\Gamma(1+w), \\
%%% \lign
%%% \hspace{5.23cm}
%%% \def\lur{\rule{1.5cm}{.4pt}}\shortmid\hspace{-.135cm}\lower.5pt\hbox{$\lur$}
%%% \hspace{-.138cm}\shortmid
%%% \end{array}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%   GRAMMH PLAGIA %%%%%%%%%%%%%%%%%
%%% \lower12pt\hbox{\hspace{-1.1cm}\rotatebox{50}{\rule{15mm}{.3pt}}}




%%%%%%%%%%%%%%%%%%% GIA GRAMMH ME PLAINA %%%%%%%%%%%%%%
%%% \noindent
%%% $\hskip5.85cm\vrule height 2 pt width 0.2 pt\hskip-.085cm$
%%% ${\vrule height 0.3pt width 0.9 cm}\hskip-.085cm$
%%% $\vrule height 2 pt width 0.2 pt$


